Polynomial-time algorithm for Maximum Weight Independent Set on $P_6$-free graphs

In the classic Maximum Weight Independent Set problem we are given a graph $G$ with a nonnegative weight function on vertices, and the goal is to find an independent set in $G$ of maximum possible weight. While the problem is NP-hard in general, we give a polynomial-time algorithm working on any $P_6$-free graph, that is, a graph that has no path on $6$ vertices as an induced subgraph. This improves the polynomial-time algorithm on $P_5$-free graphs of Lokshtanov et al. (SODA 2014), and the quasipolynomial-time algorithm on $P_6$-free graphs of Lokshtanov et al (SODA 2016). The main technical contribution leading to our main result is enumeration of a polynomial-size family $\mathcal{F}$ of vertex subsets with the following property: for every maximal independent set $I$ in the graph, $\mathcal{F}$ contains all maximal cliques of some minimal chordal completion of $G$ that does not add any edge incident to a vertex of $I$.

==> capturing-hidden.tex <==
\subsection{Easy auxiliary lemmas}

\begin{definition}
A minimal separator $S$ in $G$ is {\em{hidden}} if either $G-S$ has at least $3$ components full to $S$, or there is minimal separator $S'$ in $G$ with $S\subsetneq S'$.
\end{definition}

From Lemma~\ref{lem:pmc-minseps} we immediately obtain the following.

\begin{observation}\label{obs:hidden}
Let $\Om$ be a PMC in $G$, and a suppose there are different components $D,D'\in \cc(G-\Om)$ such that $N(D)\subseteq N(D')$. Then $N(D)$ is a hidden minimal separator in $G$.
\end{observation}

We now show that the number of hidden minimal separators is small and we can enumerate their superfamily.

\begin{lemma}\label{lem:see-hidden}
One can in polynomial time compute a family $\Ss_\hid\subseteq 2^{V(G)}$ of size at most $n^7$ that contains every hidden minimal separator in $G$.
\end{lemma}
\begin{proof}
Fix a hidden minimal separator $S$. 

Suppose first that $G-S$ has three components full to $S$, say $D_1,D_2,D_3$. Consider the graph $G'=G[D_1\cup S\cup D_2]$; certainly, $G'$ is $P_6$-free and $S$ is still a minimal separator in $G'$.
By Lemma~\ref{lem:covering-simple} there exists a set $A\subseteq D_1\cup D_2$ of size at most $6$ each such that $S\subseteq N[A]$.
Observe that $N[A]$ is disjoint from $D_3$ and contains $S$, hence we have that $S=\Proj_G(u,N[A])$ for any $u\in D_3$.

Suppose now that there is some minimal separator $S'$ such that $S\subsetneq S'$; take any $x\in S'\setminus S$. Let $D_1$ and $D_2$ be two components of $G-S'$ full to $S'$.
Since both $D_1$ and $D_2$ are adjacent to $x$, it follows that they are both contained in the same component $D'$ of $G-S$. Let $D_3$ be any component of $G-S$ that is full to $S$ and different than $D'$.
In particular, $D_3$ is disjoint from $D_1$ and $D_2$. Again, consider the graph $G'=G[D_1\cup S'\cup D_2]$, and by the same analysis as in the previous paragraph we infer that there exists
a set $A\subseteq D_1\cup D_2$ of size at most $6$ each such that $S\subseteq N[A]$. Then again $N[A]$ is disjoint from $D_3$ and contains $S$, hence again $S=\Proj_G(u,N[A])$ for any $u\in D_3$.

Consider the following procedure for computing $\Ss_\hid$: for every choice of $A\subseteq V(G)$ with $|A|\leq 6$ and $u\notin N[A]$, add the set $\Proj_G(u,N[A])$ to $\Ss_\hid$.
From the above analysis it follows that $\Ss_\hid$ constructed in this manner contains every hidden minimal separator, while $|\Ss_\hid|\leq n^7$ by the construction.
\end{proof}

\begin{definition}
For a PMC $\Om$ in $G$, by $\maxnei(\Om)$ we denote the set of those components $D\in \cc(G-\Om)$, for which there is no component $D'\in \cc(G-\Om)$ with $D'\neq D$ and $N(D)\subseteq N(D')$.
\end{definition}

Note that in the above definition, if there are two different components $D_1,D_2\in \cc(G-\Om)$ with $N(D_1)=N(D_2)$, then neither of them is contained in $\maxnei(\Om)$.
The next lemma shows that components outside of $\maxnei(\Om)$ are easy to recognize.

\begin{lemma}[cf.~Lemma~\ref{o:lem:hidden}]\label{lem:see-pmc-hidden}
One can in polynomial time compute a family $\Ff_\hid$ of size at most $n^8$ such that the following holds: for any PMC $\Om$ in $G$ and any $D\in \cc(G-\Om)$ such that $D\notin \maxnei(\Om)$,
we have $D\in \Ff_\hid$.
\end{lemma}
\begin{proof}
Consider the following procedure for constructing $\Ff_\hid$: construct the family $\Ss_\hid$ given by Lemma~\ref{lem:see-hidden}, and for each $S\in \Ss_\hid$ add $\cc(G-S)$ to $\Ff_\hid$.
To see that $\Ff_\hid$ constructed in this manner satisfies the required properties, take any PMC $\Om$ and $D\in \cc(G-\Om)$ with $N(D)\notin \maxnei(\Om)$.
Since $N(D)\notin \maxnei(\Om)$, there is some $D'\in \cc(G-\Om)$ with $D\neq D'$ and $N(D)\subseteq N(D')$, which by Observation~\ref{obs:hidden} implies that $N(D)$ is a hidden minimal separator in $G$.
By Lemma~\ref{lem:see-hidden} we have $N(D)\in \Ss_\hid$, which implies that $D\in \Ff_\hid$ because we included all connected components of $G-N(D)$ in the construction of $\Ff_\hid$.
\end{proof}

